NN-Based FeFET Compact Modeling for SPICE Simulation

Prototyping and early-stage circuit evaluation for emerging transistor technologies require fast and accurate compact models for SPICE simulations. Standard physics-based compact models, such as BSIM, offer high fidelity but demand extensive domain expertise and time-consuming equation formulation for every new physical effect, significantly slowing technology development. Neural network (NN)-based models offer a scalable alternative approach, but they rely heavily on smooth numerical solver data with explicit high-order derivative information. However, measurement data suffers from complex noise patterns, making derivative extraction challenging and complicating NN-based transistor modeling. This work presents a derivative-free NN training framework employing spectral normalization to naturally smooth derivative behavior and filter measurement noise. Using drain current measurements from a fabricated 28 nm ferroelectric device, we design an NN-based compact model that captures the full spectrum of polarization amplitudes and supports dynamic polarization switching in transient simulations. To demonstrate its capability, we deploy the model in a commercial SPICE software to simulate write and read operations for large-scale memory arrays with up to 512x512 size, including parasitic effects. Our approach bridges raw measurements with NN-based SPICE-compatible transistor modeling, significantly reducing model development time and enabling rapid circuit-level prototyping for emerging devices.

==> 1_initial/figures/memory_template.tex <==
\pgfmathsetmacro{\gridScaleX}{1.5}
\pgfmathsetmacro{\gridScaleY}{1.1}

\pgfmathtruncatemacro{\maxIdx}{\gridSize-1}
\def\stub{3}       % how far lines extend past the outermost transistor
\def\dotRadius{0.04} % radius of the connection dots

% --- Draw the FeFET grid ---
\foreach \ix in {0,...,\maxIdx}
    \foreach \iy in {0,...,\maxIdx}
        {
        \node [nmos, tr gap fill=fefetcolor, ferroel gate, anchor=D, rotate=-90]
            (mn\ix-\iy) at (\gridScaleX*\ix,\gridScaleY*\iy) {};
        }

% --- Horizontal gate lines (WL), index 0 at the top ---
\foreach \iy in {0,...,\maxIdx}
    {
    \pgfmathtruncatemacro{\wlIndex}{\maxIdx-\iy}
    \draw let \p1=(mn0-\iy.G), \p2=(mn0-\iy.D), \p3=(mn0-\iy.S),
             \p4=(mn\maxIdx-\iy.G), \p5=(mn\maxIdx-\iy.D), \p6=(mn\maxIdx-\iy.S),
             \n1={min(\x1,min(\x2,\x3))},
             \n2={max(\x4,max(\x5,\x6))}
         in
         coordinate (wl\wlIndex) at ([xshift=-\stub]\n1,\y1)
         (\n1-\stub,\y1) -- (\n2+\stub,\y1);
    }

% --- Horizontal drain lines (SL), index 0 at the top ---
\foreach \ix in {0,...,\maxIdx}
    {
    \draw let \p1=(mn\ix-0.S), \p2=(mn\ix-\maxIdx.D), \p3=(mn\ix-\maxIdx.G) in
        coordinate (sl\ix) at ([yshift=\stub]\x2,\y3)
        (\x2,\y1-\stub) -- (\x2,\y3+\stub);
    }

% --- Vertical source lines (BL), one straight line per column ---
\foreach \ix in {0,...,\maxIdx}
    \draw let \p1=(mn\ix-0.S), \p2=(mn\ix-\maxIdx.D), \p3=(mn\ix-\maxIdx.G) in
        coordinate (bl\ix) at ([yshift=\stub]\x1,\y3)
        (\x1,\y1-\stub) -- (\x1,\y3+\stub);

% --- Connection dots at every terminal of every transistor ---
\foreach \ix in {0,...,\maxIdx}
    \foreach \iy in {0,...,\maxIdx}
        {
        \fill (mn\ix-\iy.G) circle (\dotRadius);
        \fill (mn\ix-\iy.S) circle (\dotRadius);
        \fill (mn\ix-\iy.D) circle (\dotRadius);
        }
